Neural Machine Translation Inspired Binary Code Similarity Comparison beyond Function Pairs

Binary code analysis allows analyzing binary code without having access to the corresponding source code. A binary, after disassembly, is expressed in an assembly language. This inspires us to approach binary analysis by leveraging ideas and techniques from Natural Language Processing (NLP), a rich area focused on processing text of various natural languages. We notice that binary code analysis and NLP share a lot of analogical topics, such as semantics extraction, summarization, and classification. This work utilizes these ideas to address two important code similarity comparison problems. (I) Given a pair of basic blocks for different instruction set architectures (ISAs), determining whether their semantics is similar or not; and (II) given a piece of code of interest, determining if it is contained in another piece of assembly code for a different ISA. The solutions to these two problems have many applications, such as cross-architecture vulnerability discovery and code plagiarism detection. We implement a prototype system INNEREYE and perform a comprehensive evaluation. A comparison between our approach and existing approaches to Problem I shows that our system outperforms them in terms of accuracy, efficiency and scalability. And the case studies utilizing the system demonstrate that our solution to Problem II is effective. Moreover, this research showcases how to apply ideas and techniques from NLP to large-scale binary code analysis.

==> table-bak.tex <==


\begin{comment}
\begin{table*}
\footnotesize
\caption{Examples of semantically equivalent basic blocks that are correctly classified by \bbtool, but misclassified by the
statistical feature-based SVM model.}\label{table:block_examples}
\af
\centering
\renewcommand{\arraystretch}{1.07}
\scalebox{0.96}{
\begin{tabular}{@{}l@{}|@{~}l@{}V{2.5}@{~}l@{}|@{~}l@{}V{2.5}@{~}l@{}|@{~}l@{}}
\hline
%original & equivalent & original & equivalent\\\hline
\multicolumn{2}{cV{2.5}}{\textbf{Pair 1}} & \multicolumn{2}{cV{2.5}}{\textbf{Pair 2}}  & \multicolumn{2}{c}{\textbf{Pair 3}} \\ \hline
\multicolumn{1}{c|}{\emph{x86}}  & \multicolumn{1}{cV{2.5}}{\emph{ARM}}  & \multicolumn{1}{c|}{\emph{x86}} & \multicolumn{1}{cV{2.5}}{\emph{ARM}} & \multicolumn{1}{c|}{\emph{x86}} & \multicolumn{1}{c}{\emph{ARM}}   \\
\hline
       CALLQ FOO              & BL FOO         & ANDL R12D, 0   & LDR R8, [SP+0]   &  XORL EBX, EBX    & CMP R4, 0 \\
       MOVQ [RIP+<TAG>], RAX  & STR R0, [R7]   & JE <TAG>       & ANDS R1, R0, 0   &  TESTL EBP, EBP   & BLT <TAG> \\
       TESTQ RAX, RAX         & CMP R0, 0      &                & BEQ <TAG>        &  JS <TAG>         &  \\
       JE <TAG>               & BEQ <TAG>      &                &                  &   &  \\

\hhline{==V{2.5}==V{2.5}==}
%\hline
%\clineB{1-6}{2.5}
\multicolumn{2}{cV{2.5}}{\textbf{Pair 4}} & \multicolumn{2}{cV{2.5}}{\textbf{Pair 5}} &  \multicolumn{2}{c}{\textbf{Pair 6}} \\ \hline
\multicolumn{1}{c|}{\emph{x86}}  & \multicolumn{1}{cV{2.5}}{\emph{ARM}}  & \multicolumn{1}{c|}{\emph{x86}} & \multicolumn{1}{cV{2.5}}{\emph{ARM}} & \multicolumn{1}{c|}{\emph{x86}} & \multicolumn{1}{c}{\emph{ARM}}   \\
\hline
PUSHQ R14          & PUSH \{R4, R5, R11, LR\} & MOVQ EAX, R13D  & MOV R0, R6                  & MOVQ RAX, <TAG>+[RIP+0]  & LDR R0, <TAG>   \\
PUSHQ RBX          & MOV R4, R0               & ADDQ RSP, 0     & ADD SP, SP, 0               & CMPQ RAX, [RSP+0]        & LDR R1, [R0+0] \\
PUSHQ RAX          & LDR R0, [R4+0]           & POPQ RBX        & POP \{R4,R5,R6,R7,R11,LR\}  & JNE <TAG>                & LDR R2, [R0+0] \\
MOVQ RBX, RDI      & LDRB R2, [R0]            & POPQ R12        & MOV PC, LR                  &                          & LDR R3, [SP+0] \\
MOVQ RAX, [RBX+0]  & CMP R2, 0                & POPQ R13        &                             &                          & LDR R7, [SP+0] \\
CMPB [RAX], 0      & BNE <TAG>                & POPQ R14        &                             &                          & EOR R2, R2, R7 \\
JNE <TAG>          &                          & POPQ R15        & 		              &                          & EOR R1, R1, R3 \\
		   &			      & RETQ            & 		              &                          & ORRS R1, R1, R2 \\
		   &			      &                 & 		              &                          & BNE <TAG> \\
 
\hline
\end{tabular}
}
\af
\end{table*}
\end{comment}

